The Black-Box Simplex Architecture for Runtime Assurance of Autonomous CPS

The Simplex Architecture is a runtime assurance framework where control authority may switch from an unverified and potentially unsafe advanced controller to a backup baseline controller in order to maintain the safety of an autonomous cyber-physical system. In this work, we show that runtime checks can replace the requirement to statically verify safety of the baseline controller. This is important as there are many powerful control techniques, such as model-predictive control and neural network controllers, that work well in practice but are difficult to statically verify. Since the method does not use internal information about the advanced or baseline controller, we call the approach the Black-Box Simplex Architecture. We prove the architecture is safe and present two case studies where (i) model-predictive control provides safe multi-robot coordination, and (ii) neural networks provably prevent collisions in groups of F-16 aircraft, despite the controllers occasionally outputting unsafe commands.

==> Sections/acasxu_discussion.tex <==
\subsubsection{Discussion}

The acceptance condition for \dmupdate checked by the decision module consists of three parts described earlier: (i)~the system state stays within model limits, (ii)~the horizontal safety distance is maintained at all times, and (iii)~the maneuver ends with straight-and-level flight, with all aircraft moving away from each other.
%
However, there are many behaviors we would want to avoid that are \emph{not} checked by this logic.
%
For example, flying into the ground will not cause a command sequence to be rejected.
%
The system could also command maximum afterburner, which would waste fuel unnecessarily, or actuate the system wildly in ways that would damage a real airframe or cause excessive wear.
%
We could try avoid these cases by enumerating them and adding appropriate checks in the decision module.
%
However, the possibilities for misbehavior are large, and such an approach is likely to miss undesirable cases.
%
Note that this problem is not unique to Black-Box Simplex, but also exists with the original Simplex Architecture.
%
Another way to address this issue is to push it aside---assume that although the controllers are unverified, they are not malicious and so the decision module can focus on checking the aspects of the controllers that are most critical and more likely to be incorrect.

A third---perhaps better---way to handle this issue is to reformulate the problem. 
%
We can modify the ``Plant + Low-Level Controller'' box in Black-Box Simplex to also include trusted low-level controllers for the following six actions: (1)~fly towards the waypoint, (2)~fly straight, (3)~turn weak left, (4)~turn weak right, (5)~turn strong left, and (6)~turn strong right.
%
At each decision point, then, the advanced controller always chooses the first action, whereas the baseline controller's ACASXu system produces an output corresponding to one of the latter five actions, for each aircraft.
%
Creating a reliable controller individually for each of these six actions is much closer to a classical control problem; we could assume such controllers are provided that can maintain altitude and airspeed and do not fly into the ground or damage the aircraft in other ways.
%
The problem solved by Black-Box Simplex is then about \emph{high-level} control: how to safely compose these actions to reach the target waypoint while maintaining the safety constraint.
%
%Viewed in this way, the controllers that choose among these actions can truly be treated as black boxes that may even be malicious.

Another limitation of this case study is that it does not have disturbances, so the dynamics are deterministic.
%
Handling disturbances with the same approach as in the previous case study, using online reachability computation, would be difficult for several reasons.
%
First, closed-form differential equations---which are required by most reachability tools---are not provided for this system, as the derivative is computed by Python code.
%
It would be hard to even extract differential equations from the code, as the simulator includes components like multiple look-up tables and conditional branches.
%
Second, the simulation has nonlinear dynamics, for which reachability methods scale more poorly than with linear dynamics.
%
Third, the number of variables can be large, for example 240 real-valued state variables in the 15-aircraft case.
%
This complexity of system is beyond what is currently possible with nonlinear reachability tools~\cite{geretti2020arch}, and even if it becomes possible, it is unlikely to run fast enough for use at runtime.

Instead, the more feasible approach would again be to rely on control theory to provide performance guarantees for the designed controllers.
%
If each maneuver resulting from the six actions described earlier could be analyzed for maximum overshoot and steady-state error---typical metrics evaluated during control design---executions of the system could be computed and then bloated by the worst-case distance to obtain a lower bound on the minimum horizontal separation.
%
Used like this, Black-Box Simplex builds upon the vast body of work from control theory to produce safe high-level behaviors from untrusted controllers.

In terms of the runtime of the decision module simulation logic, we have not yet optimized its computation time in our implementation.
%
Importantly, since each aircraft's dynamics are disjoint, there is significant room for speedup through parallelism, up to the number of aircraft in the system.
%
The existing implementation simulates the dynamics using an adaptive-step explicit Runge-Kutta scheme of order 5(4) from Python's \texttt{scipy} package.
%
On our laptop platform with default accuracy parameters, this runs at about 55 times faster than real-time per aircraft.
%
As future work, we could consider optimizing runtime by using different numerical integration strategies, depending on factors such as the distance to the safety violation.
